Finite Automata for Efficient Graph Recognition

Engelfriet and Vereijken have shown that linear graph grammars based on hyperedge replacement generate graph languages that can be considered as interpretations of regular string languages over typed symbols. In this paper we show that finite automata can be lifted from strings to graphs within the same framework. For the efficient recognition of graphs with these automata, we make them deterministic by a modified powerset construction, and state sufficient conditions under which deterministic finite graph automata recognize graphs without the need to use backtracking.

==> eptcsdata.tex <==
\providecommand{\firstpage}{134}
\providecommand{\publicationstatus}{J. Endrullis, D. Grzelak, T. Heindel and J. Kosiol (Eds):\\ GCM 2023 and GCM 2024\\
EPTCS 417, 2025, pp.\ \pageref*{FirstPage}--\pageref{LastPage},
doi:\href{http://dx.doi.org/10.4204/EPTCS.417.8}{10.4204/EPTCS.417.8}}
\pdfoutput=1

